Towards Human-Understandable Multi-Dimensional Concept Discovery

Concept-based eXplainable AI (C-XAI) aims to overcome the limitations of traditional saliency maps by converting pixels into human-understandable concepts that are consistent across an entire dataset. A crucial aspect of C-XAI is completeness, which measures how well a set of concepts explains a model's decisions. Among C-XAI methods, Multi-Dimensional Concept Discovery (MCD) effectively improves completeness by breaking down the CNN latent space into distinct and interpretable concept subspaces. However, MCD's explanations can be difficult for humans to understand, raising concerns about their practical utility. To address this, we propose Human-Understandable Multi-dimensional Concept Discovery (HU-MCD). HU-MCD uses the Segment Anything Model for concept identification and implements a CNN-specific input masking technique to reduce noise introduced by traditional masking methods. These changes to MCD, paired with the completeness relation, enable HU-MCD to enhance concept understandability while maintaining explanation faithfulness. Our experiments, including human subject studies, show that HU-MCD provides more precise and reliable explanations than existing C-XAI methods. The code is available at https://github.com/grobruegge/hu-mcd.

==> sec/3_proposed_method_old.tex <==
\section{Proposed Method}

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/method_overview.pdf}
    \caption{Overview of HU-MCD.}
    \label{fig:method_overview}
\end{figure*}

% As outlined by~\citet{fel2024holistic}, the majority of existing automatic concept-based explanation methods share two fundamental stages: (1) concept discovery, involving the extraction of concepts from a corpus of training images,  typically belonging to the same class, and (2) concept importance scoring, aimed at quantifying the influence of each concept on the final classifier (class) prediction.

Building on the goals of discovering human-\textit{understandable} concepts and \textit{faithfully} attribute their contribution to the model's prediction strategy, we propose Human-Understandable Multi-Dimensional Concept Discovery (HU-MCD). As shown in
Figure~\ref{fig:method_overview}, we distinguish two stages for HU-MCD to align
with existing literature~\citep{fel2024holistic}. First, we discover relevant concepts by segmenting class images using SAM~\citep{kirillov2023segment}, a foundation model for instance segmentation. We cluster them using SSC based on their representation within the feature space of the model. To avoid introducing noise that distort the model's prediction by rescaling and inpainting image segments, we employ an input masking scheme specifically designed for CNNs~\citep{balasubramanian2023towards}. Second, we adapt the MCD framework proposed by~\citet{vielhaben2023multi} which allows for both local and global concept importance scoring and incorporates a completeness relation by decomposing the model's feature space into multi-dimensional concepts.

% In the following subsections we are going to describe the individual phases of HU-MCD in detail.

\subsection{Concept Discovery} 

We chose a set of images that encapsulate the concepts against which the model will be tested. The selection of samples is not constrained, giving users the flexibility to choose class-specific samples or utilize the entire training set to derive class-agnostic concepts. Inspired by ACE, we use a segmentation algorithm to obtain a dataset comprising distinct image regions acting as concept candidates. In particular, we use SAM~\citep{kirillov2023segment}. SAM's utility to perform precise and comprehensive instance segmentation and its ability for zero-shot generalization have been demonstrated across a broad spectrum of tasks, including XAI~\citep{sun2024explain}. Using the masks provided by SAM, we select, for each image, the most granular decomposition, considering all masks covering at least $1\%$ of the image.

% SAM offers several advantages, including the ability to provide human-understandable segmentation masks, automatically determine segmentation parameters, and handle ambiguity in segmentation tasks by providing multiple masks at varying depths. I aim to achieve a distinct decomposition of images into different segments, ensuring that each part of the image is uniquely assigned a concept later on.

\noindent
We cluster perceptually similar segments within the candidate dataset as entities of the same concept. Concepts are inherently linked to the hidden representation of intermediate feature layers. Previous work has demonstrated that state-of-the-art CNNs learn to represent different features of the data by mapping distinct concepts to different regions of the embedding space~\citep{zhang2018unreasonable}. We thus use SSC to ensure that all data points within different clusters lie on a union of distinct low-dimensional subspaces embedded within a higher-dimensional space, as outlined by \citet{vielhaben2023multi}, effectively grouping similar segments. Instead of opting for an arbitrary cluster count, as seen in prior studies (\eg, 10~\citep{zhang2021invertible} or 25~\citep{ghorbani2019towards, fel2023craft}), we leverage the robust segmentation capabilities of SAM and determine the number of clusters based on the average number of segments per image.\looseness=-1

\noindent
How to pass the resulting irregular-shaped regions through CNN models and obtain the feature embeddings is non-trivial; the fixed-size input expectation of CNN architectures requires rescaling and/or the incorporation of baseline colors to fill the masked-out regions, as done by ACE. However, since many of these baseline colors are not truly neutral~\citep{jain2022missingness}, these manipulations can introduce noise that is picked up by the model during inference. To address this problem, approaches such as classical imputation algorithm~\citep{bertalmio2001navier}, as suggested by~\citet{vielhaben2023multi}, have been proposed. Despite this, these methods may still introduce \textit{missingness bias}---the model reveals hidden information by recovering masked-out regions.
% which can be expensive.
\citet{balasubramanian2023towards} have thus proposed a layer masking scheme for CNNs; instead of replacing the masked regions with a baseline color, they propagate both the input image and the mask at each layer. This is achieved by leveraging the hierarchical architecture of CNNs, which consists of stacked convolutional layers that gradually increase their receptive field. As such, at each layer, the masking scheme retains values dependent only on the unmasked input while discarding those reliant solely on the masked region.

% To the best of our knowledge, we are the first to apply Layer Masking to concept-based explanations.

% Discuss how to handle edge convolutions?

\subsection{Concept Importance Scoring} 

To quantify the importance of concepts in influencing specific class predictions, we adopt the concept decomposition framework proposed by~\citet{vielhaben2023multi} because it incorporates a completeness relation, distinguishing it from alternative methods.

\noindent
As stated previously, concepts are inherently linked to shared patterns in the activation space of neural networks. Given an input image $x$, the model $f$ is split into two parts, $f(x) = g(h(x))$, where $h(x) := \bm{\phi} \in {\mathbb{R}}^{D}$ is the mapping to the hidden $D$-dimensional feature layer\footnote{Vectors are denoted in bold}, which is then mapped to the final prediction by $g(\bm{\phi})$. Concept-based explanations aim to determine the properties (\ie, concepts) of $x$ that influence the prediction $f_k(x)$ of a given class $k$ \citep{zhou2018interpretable}. To this end, the feature space (union of all possible activation in ${\mathbb{R}}^{D}$) is decomposed into concepts that are mathematically formalized as multi-dimensional linear subspaces of arbitrary dimensionality. 

\noindent
Following the concept discovery procedure, for a given class $k$, we identify $n$ clusters $\mathcal{C}^1, \dots,\mathcal{C}^n$ represented by image segments mapped to the hidden feature layer. Next, we want to become independent of the original cluster members and find a representative basis $C^l$ that disentangles frequently appearing activation patterns within the cluster $\mathcal{C}^l$. SSC ensures that cluster members $\bm{\phi}_i \in \mathcal{C}^l$ lie within a linear subspace embedded into the high-dimensional feature space ${\mathbb{R}}^{D}$. This makes PCA a suitable linear tool to construct a concept basis $C^l$ for cluster $\mathcal{C}^l$. The top principal components up to an intrinsic dimension $d_l$ serve as basis vectors $\bm{c}_{i}^{l}$ for $i=0,\ldots,d_l$ for the subspace spanned by $C^l$. We determine the intrinsic dimension as minimal principal components required to preserve $80\%$ of the variance. Repeating this process for every cluster results in $n$ concept bases ${C}^1, \dots, {C}^n$, which represent frequently appearing patterns given a class $k$. To ensure that the union of all concept subspaces spans the entire feature space, \citet{vielhaben2023multi} propose to calculate the orthogonal complement of the subspace spanned by all concepts, i.e., $C^{n+1} = span(C^1, \dots, C^n)^{\perp}$. 

% This assumes that the concept subspaces are pairwise disjoint which is usually not violated but could be enforced by removing the intersections and considering them as separate concepts.

\noindent
This setup allows the decomposition of any feature vector $\bm{\phi}$ from a given image into its concept contribution. \citet{vielhaben2023multi} propose two complementary tools to evaluate samples locally: \textit{concept activation}, which highlights the presence of a concept, and \textit{concept relevance}, which indicates the impact of a concept on the model's prediction. On a global level, they propose the \textit{global concept relevance score}, which demonstrates the overall impact of concepts on class predictions. 

\noindent\textbf{Concept Activations} indicate the presence of each concept in a feature vector $\bm{\phi}$. This is realized by decomposing $\bm{\phi}$ into its unique concept attributions as

\begin{equation}
        \bm{\phi} = \sum_{l=1}^{n+1} \sum_{i=1}^{d_{l}} \varphi_{i}^{l} \bm{c}_{i}^{l} \equiv \sum_{l=1}^{n+1} \bm{\phi}^{l},
\end{equation}

\noindent
where $\varphi_{i}^{l}$ are the coefficients by which the basis vectors $\bm{c}_{i}^{l}$ of each concept basis $C^l$ are weighted for each decomposition. Essentially, $\bm{\phi}^{l}$ represents the projection of $\bm{\phi}$ onto the concept subspace spanned by $C^l$. The expressiveness of concept $l$ can be interpreted as the proportion of the feature vector $\bm{\phi}$'s magnitude attributable to each concept $\| \bm{\phi}^{l} \| / \|\bm{\phi}\|$ where $\|\cdot\|$ denotes the Euclidean norm. By repeating this process for the latent feature vector of every segment within an image, each region can be associated with concept activation scores, effectively creating a \textit{concept activation maps} in the input space. We sort test samples in descending order of concept activation and choose the maximally activating samples as \textit{concept prototypes}.

\noindent
Concept activations indicate which concepts are strongly present within an image but do not give any insights into the extent (positively or negatively) these concepts influence the model's prediction. To this end, we define $h$ up to the final hidden layer within a CNN (after the pooling operation), only followed by the linear classification head $g$. 

\noindent\textbf{Concept Relevance} quantifies the impact of a concept on the classification decision. As defined above, $g$ only consists of a linear classification head; thus for a given class, the weight vector $\bm{w} \in {\mathbb{R}}^{D}$ linearly connects the $D$-dimensional feature space $h(x) \in {\mathbb{R}}^{D}$ with the scalar class prediction. This allows to decompose the class logit $\bm{\phi} \cdot \bm{w} + b$ up to the bias term as

\begin{equation}
    \label{eq:relevance_decomposition}
    \bm{\phi} \cdot \bm{w} = \sum_{l=1}^{n+1} \bm{\phi}^{l} \cdot \bm{w} \equiv \sum_{l=1}^{n+1} {r}^{l}
\end{equation}

\noindent
This decomposition defines a \textit{local concept relevance} score. Aggregating relevance scores ${r}^{l}$ from all concepts recovers the class logit prediction (up to the bias term), and thus, Equation~\ref{eq:relevance_decomposition} defines a \textit{completeness} relation. In the same fashion as for concept activations, we can define \textit{concept relevance maps} by computing the local concept relevance for each segment. 

\noindent\textbf{Global concept relevance scores} evaluate the overall impact of concepts on class prediction. Because the union of all concept basis vectors $\bm{c}^l_j$ (including the orthogonal complement) defines a basis for the feature space ${\mathbb{R}}^{D}$, \citet{vielhaben2023multi} propose to decompose the final class weight vector $w$ into 

\begin{equation}
    \bm{w} = \sum_{l=1}^{n+1} \sum_{i=1}^{d^l} w_i^l \bm{c}_i^l \equiv \sum_{l=1}^{n+1} \bm{w}^l
\end{equation}

\noindent
where $\bm{w}^l$ is the projection of the class vector into the concept subspace spanned by the basis $C^l$. To quantify the global concept importance and define a completeness score, one can decompose the squared Euclidean norm $\|\bm{w}\|^2$ into the concept attributions. Given the definition of orthogonality, i.e., $\bm{w}^l \cdot \bm{w}^{\perp} = 0$ $\forall l \in \{1,...,n\}$, we have

\begin{equation}
    \|\bm{w}\|^2 = \| \bm{w}^{\perp} \|^2 + \| \sum_{l=1}^{n} \bm{w}^l \|^2 
\end{equation}

\noindent
Hence, the completeness score can be defined as the fraction of $\bm{w}$, which is explained by all concepts $\{C^1,...,C^n\}$ with respect to a given class.

\begin{equation}
\label{eq:weight_vector_decomposition}
    \eta(\{C^l\}) = 1 - \frac{\| \bm{w}^{\perp} \|^2}{\| \bm{w} \|^2}
\end{equation}

\noindent
Given that the corresponding minimal and maximal principal angles define bounds for $\| \bm{w} \|^2$, we can interpret $\| \bm{w^l} \|^2 / \| \bm{w} \|^2 $ as global relevance scores. We omit the details here and refer to the more detailed description by \citet{vielhaben2023multi}. Overall, the completeness is impacted by adapting concept discovery parameters such as concept subspaces or the number of clusters. For instance, increasing the number of clusters could lead to higher completeness while reducing the subspaces (e.g., principal components of concepts) could decrease completeness.

% In case the concept subspaces are restricted to be orthogonal to each other, the second term in the last equality of  Equation~\ref{eq:weight_vector_decomposition} (cosine) disappears, hence $\| \bm{w^l} \|^2 / \| \bm{w} \|^2 $ directly sum up to the completeness score and can be interpreted as global relevance score. However, \citet{vielhaben2023multi} show that this leads to less faithful concept representation which is why it is not enforced when creating the concept bases. The subspace angles in Equation~\ref{eq:weight_vector_decomposition} are bounded by the corresponding minimal and maximal principal angles, which allows to define lower and upper bounds for $\| \bm{w} \|^2$ and implies that $\| \bm{w^l} \|^2 / \| \bm{w} \|^2 $ are also informative in the non-orthogonal case. We omit the details here and refer to the more detailed description by \citet{vielhaben2023multi}.

